On Advances in Text Generation from Images Beyond Captioning: A Case Study in Self-Rationalization

Combining the visual modality with pretrained language models has been surprisingly effective for simple descriptive tasks such as image captioning. More general text generation however remains elusive. We take a step back and ask: How do these models work for more complex generative tasks, i.e. conditioning on both text and images? Are multimodal models simply visually adapted language models, or do they combine they reason jointly over modalities? We investigate these questions in the context of self-rationalization (jointly generating task labels/answers and free-text explanations) of three tasks: (i) visual question answering in VQA-X, (ii) visual commonsense reasoning in VCR, and (iii) visual-textual entailment in e-SNLI-VE. We show that recent unimodal advances, CLIP image representations and scaling of language models, do not consistently improve self-rationalization in multimodal tasks. We find that no single model type works universally best across tasks, datasets, and finetuning data sizes. Our findings motivate the need for novel general backbones approach that move text generation from images and text beyond image captioning.

==> sections/abstract.tex <==


Integrating vision and language has gained notable attention following the success of pretrained language models. %
Despite that, a fraction of emerging multimodal models is suitable for \emph{text generation} conditioned on images. %
This minority is typically developed and evaluated for image captioning, a text generation task conditioned solely on images with the goal to describe what is explicitly visible in an image. %
In this paper, we take a step back and ask: How do these models work for more complex generative tasks, conditioned on both text and images? %
Are models based on joint multimodal pretraining, visually adapted pretrained language models, or models that combine these two approaches, more promising for such tasks? %
We address these questions in the context of \emph{self-rationalization} (jointly generating task labels/answers and free-text explanations) of three tasks: (i) visual question answering in \vqax, (ii) visual commonsense reasoning in \vcr, and (iii) visual-textual entailment in \esnlive. %
We show that recent advances in each modality, CLIP image representations and scaling of language models, do not consistently improve multimodal self-rationalization of tasks with multimodal inputs. % 
We also observe that no model type works universally the best across tasks/datasets and finetuning data sizes. %
 Our ﬁndings call for a backbone modelling approach that can be built on to advance text generation from images and text beyond image captioning. 

==> sections/conclusions.tex <==
We analyze model instances from distinct model families that we expect to have unique benefits and downsides for text generation conditioned on images and text beyond image captioning. % 
We evaluate them for self-rationalization (jointly generating labels/answers and free-text explanations) of three multimodal tasks. %
We observe that model scaling and latest image representations do not clearly improve visually adapted pretrained language models. 
Our main finding is that a single model (family) does not work universally the best across tasks and available finetuning data. %
Future advances in text generation conditioned on images and text should be demonstrated using a variety of tasks/datasets and dataset sizes, and researchers should develop a method that realizes all the benefits of different model families.

==> sections/related_work.tex <==
\ana{Not complete?} 

\citeauthor{Dua2021BeyondVG} \citeyear{Dua2021BeyondVG} propose \textit{Beyond VQA} the task of generating multi-word answers and rationales to visual questions. This was one of the first papers that propose to generate both the answer, and the rationale for a given question-image pair.\ana{This is not precise, they are not the first to propose this \cite{hendricks2016generating, kim2018textual, hancock-etal-2018-training, camburu2018snli, ehsan2018rationalization, liu-etal-2019-towards-explainable, wu-mooney-2019-faithful, narang2020wt5, tang-etal-2020-exploring, wiegreffe-etal-2021-measuring, Kayser2021eViLAD}. They are the first to propose generating answers for VCR.}  The task of visual question answering \cite{Park2018MultimodalEJ}, or even providing explanations for visual questions has been explored extensively as a classification problem \cite{Zellers2019FromRT}.


There has been prior work that either assumed access to groundtruth answers for rationale generation \cite{marasovic-etal-2020-natural,Dua2021BeyondVG} or predicted answers as a classification task \cite{Kayser2021eViLAD}.

\ana{When describing Kayser et al. point to their results in the appendix and justify why we do not compare to them.}





==> sections/results_unified_vs_adapted.tex <==
We turn to our main comparison between a joint model (VLP), a visually adapted PLM (VA-T5-CLIP), and  combined models (VL-BART, VL-T5). %
Given that joint models might be advantageous when finetuning data is limited, we compare the models when  finetuned with: (i) the entire training sets (high-resource data setting), and (ii) 30\% of the training data (low-resource data setting). 


\paragraph{Results} 

In a high-resource setting (see Table \ref{tab:main_comparison_high_resource}), the best \emph{answer} accuracy/plausibility is achieved by a different model for each dataset. %
To illustrate, VA-T5 (a visually adapted PLM) obtains the best VCR answer proxy accuracy, VLP (a joint model) VCR answer plausibility, VL-T5 (a combined model) E-SNLI-VE accuracy, and VL-BART (another combined model) VQA-X accuracy. %

Explanation plausibility results are slightly more consistent (see Table \ref{tab:main_comparison_high_resource}). %
Namely, VL-BART generates most plausible explanations for E-SNLI-VE and VQA-X, and is only behind VLP for VCR. %
The best explanation BERTscore is also achieved with VL-BART for all tasks. %
However, the relative order of model types (joint, visually adapted, combined) across tasks is still mixed. %
Specifically, for VCR: joint > combined (both) > adapted (all); for E-SNLI-VE: combined (both) > adapted (all) > joint; for VQA-X: combined > adapted > joint > adapted > combined > adapted. %
Moreover, future work should consider investigating how its performance changes when other image features are used during finetuning since one advantage of visually adapting PLMs is the ability to plug and play with recent advances in representation learning of both modalities.

It is not necessarily concerning that the results are mixed given the unique benefits and downsides of these models (see Table \ref{tab:open_research_questions}) that could be relevant for one task and not another. %
However, observed cross-task differences in results are not intuitive. %
For example, visually adapting T5 and combined models give worse VCR answer and explanation plausibility compared to plausibility obtained with the joint model, VLP. %
Since generating VCR answers and explanations require the most commonsense and word knowledge relative to the other two tasks, it is reasonable to expect that this is a scenario where long pretraining on a more complex text will be beneficial, but it turns out it is not. 

We now turn to results in low-resource data setting (see Table \ref{tab:main_comparison_low_resource}). %
We hypothesized that joint models might work better when finetuning data is limited since there might not be enough images to appropriately visually adapt PLMs and they might still behave like (unimodal) language models. %
However, VA-T5 is not always underperforming relative to VLP, VL-BART, and VL-T5 in the low-resource setting. %
Specifically, VA-T5 is slightly better for explanation generation compared to VL-BART and VL-T5 for VCR, comparable to VLP for E-SNLI-VE, and better than all of the three models for VQA-X. %
It is also better than VLP for generating VCR answers. %
These results show that the size of finetuning data is not as detrimental for visual adaptation relative to joint models as we speculated.  

As in the high-resource setting, we observe that no model (type) works universally the best. %
Model ordering according to their performance sometimes stay consistent compare to the high-resource setting, e.g., for E-SNLI-VE accuracy, and sometimes changes notably, e.g., VLP gives the best VCR answer and explanation plausibility in high-resource setting, but the worst when data is limited. %
These results highlight the necessity to compare models, not only using a variety of tasks/datasets, but also models finetuned with different amounts of data.

We see that the differences between model performance in high-resource are smaller than in low-resource, where in some cases the gap is huge. %
For example, VL-BART achieves VCR answer plausibility of 42.8 in low-resource, while VLP results in only 21.1. %
Another example is VQA-X answer accuracy for which VL-BART achieves 85.6 and VLP 71.8. %
Unlike the previous example (VCR), this can be explained by the fact that VQA is one of the tasks used to pretrain VL-BART (and VL-T5). 
Such huge differences between models are not observed for explanation generation, so even though a model is much more accurate, the plausibility of explanations for its correct answers are not that much more plausible compared to explanations of other models. 


==> sections/vl_self-rationalization.tex <==
In this section, we describe tasks, datasets, and evaluation setup for self-rationalization of vision-and-language tasks introduced in prior work \cite{marasovic-etal-2020-natural, Kayser2021eViLAD}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Tasks and Datasets} 

The dataset statistics are given in Table \ref{tab:dataset_stats}, where the average answer and explanation lengths hint on differences in complexities of each task. The three datasets represent different levels of required reasoning (see examples in Figure \ref{fig:illustration}), e.g., are the images representing simpler scenarios (Flickr30K) or complex movie scenes (VCR).

\noindent \textbf{\vqax \cite{Park2018MultimodalEJ}} is the extension of the widely-used Visual Question Answering v1 \cite{antol2015vqa} and v2 \cite{goyal2017making} datasets, with corresponding free-text explanations. The images here are originally sourced from the MSCOCO dataset \cite{lin2014microsoft}, and the answers are collected for open-ended questions about these images that require vision, language, and commonsense knowledge to answer. 

\noindent \textbf{\esnlive \cite{Kayser2021eViLAD}} is a dataset for visual-textual entailment, the task of predicting whether a statement is entailed, contradicted, or neutral given an image that serves as a premise. %
\esnlive combines annotations from two datasets: (i) SNLI-VE \cite{xie2019visual}, collected by replacing the textual premises of SNLI \cite{bowman-etal-2015-large} with Flickr30K images \cite{young-etal-2014-image}, and (ii) E-SNLI \cite{camburu2018snli}, a dataset of crowdsourced free-text explanations for SNLI. %

\noindent \textbf{\vcr \cite{Zellers2019FromRT}} is a carefully crowdsourced dataset of answers and explanations for visual scenes extracted from Hollywood movies. %
Thus, the visual context in this data is more complex than MSCOCO or Flickr30K images, leading to more complex answers and explanations. %
\citeauthor{Zellers2019FromRT} instructed crowdworkers to first annotate answers for a given question-image pair, and then showed the annotated answer along with the question-image pair to a different set of annotators to get the corresponding explanation. %
This dataset was orginally introduced in a classification setting: given a question about an image, pick the correct answer from four choices, and then pick the correct explanation again from four choices. %
\citet{Dua2021BeyondVG} propose instead to generate both the answer and explanation. %
This is more realistic than the multiple-choice setting which is restricted to a user giving answer choices. %
In this paper, we also generate VCR answers and explanations.

  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Evaluation Metrics} 
\label{subsec:eval_metrics}

Self-rationalization requires evaluating two sub-tasks: correctness of predicted answers/labels, and quality of generated explanations. %
For the former, we use \textbf{accuracy} for E-SNLI-VE and VQA-X. %
Evaluating VCR answers is more complicated as they are full sentences. %
Following \citet{Dua2021BeyondVG}, given a generated answer, we normalize text (remove articles, punctuation, lowercase), and count the number of overlapping words with the four available answer choices in the VCR dataset. %
We select an answer candidate with the highest overlap as the predicted answer. %
\textbf{Proxy accuracy} is the accuracy that is computed between the correct answer candidate and predicted answer candidate. % w
\citet{Dua2021BeyondVG} do not report the correlation between proxy accuracy and human judgments of answer plausibility. %
To this end, for 600 VCR instances, we ask 5 crowdworkers to respond to ``Given the image and the question, is this answer likely?'' with yes, weak yes, weak no, or no, and map answers to 1, 2/3, 1/3, and 0, respectively. 
\textbf{Answer plausibility} is the average of scores of 5 annotators. 
In \sect{sec:results}, we report the average answer plausibility across 600 instances, as well as proxy accuracy.
Spearman's correlation coefficient between the proxy accuracy and answer plausibility is 0.56 (p < 0.028) indicating a moderate correlation between them.

Due to unreliability of automatic evaluation measures, human evaluation has been used to evaluate free-text explanation generation \cite{camburu2018snli,Kayser2021eViLAD,clinciu-etal-2021-study}. 
We ask 3 annotators whether an explanation justifies an answer/label given an image, questions/hypothesis, and a generated answer/label. %
Annotators can again pick one of the four options (yes, weak yes, weak no, no), and the four options are assigned numerical values (1, 2/3, 1/3, 0). %
We average scores of 3 annotators to get the plausibility of an individual explanation, and report the average \textbf{explanation plausibility} in a sample of 300 instances. %
Following \citet{Kayser2021eViLAD}, we select the first 300 instances for which the answer/label is correctly generated. %
For \esnlive, we select an equal number of examples for each label to produce a balanced evaluation set. 

We perform all human evaluation using Amazon Mechanical Turk. %
Each batch of evaluation contains 10 samples. %
We pay \$1.5 per batch to each annotator for \vcr evaluations and \$1 per batch for \esnlive and \vqax each as \vcr tasks require longer time to complete. %

\citet{Kayser2021eViLAD} report that all automated metrics are weakly correlated with explanation plausibility (per humans), but that BERTscore is most correlated. 
Therefore, we report \textbf{BERTscores} for completeness and reproducibility. % 
Following \citet{Kayser2021eViLAD}, we set the BERTscore of incorrectly predicted instances to 0. 

==> tables/open_research_questions.tex <==
\begin{table*}[t]
\small
\centering
\resizebox{\textwidth}{!}{  
\begin{tabular}{l|lp{15cm}}
\toprule
\multicolumn{3}{l}{\textbf{Visually Adapted PLMs:} Finetuned language models (pretrained only with text) with image features} \\
\midrule
\multirow{6}{*}{\emph{\color{mygreen} Pros}}  & 1. & Available PLMs are much larger than joint VL models. This is beneficial since text generation improves with model size \cite{brown2020gpt3}, incl.\ self-rationalization \cite{marasovic2022feb}. \\ 
& 2. & Due to huge pretraining corpora, PLMs have been shown to capture some world \cite{petroni-etal-2019-language} and commonsense knowledge \cite{davison-etal-2019-commonsense} which is beneficial for self-rationalization as it often requires \emph{inferring} relevant information from the inputs (see Fig.\ \ref{fig:illustration}). \\
& 3. & Easy to plug and play latest PLMs and image representations as there is no training from scratch. \\
\midrule
\multirow{3}{*}{\emph{\color{myred} Cons}}   & 1.  & Visual information may get suppressed, especially when finetuning multimodal data is limited. \\
& 2. & The number of images in finetuning datasets is much smaller than in pretraining multimodal datasets (e.g., Conceptual Captions with 3.3M image-caption pairs vs.\ $\sim$80K images in \vcr). \\
\bottomrule
\toprule
\multicolumn{3}{l}{\textbf{Joint VL Models:} Models based on joint pretraining of visual and textual features}   \\ 
\midrule
\multirow{3}{*}{\emph{\color{mygreen} Pros}}      &1. & Joint pretraining from scratch allows the model to learn equally from each modality without starting with any priors. Thus, this joint pretraining should give tighter coupling between modalities.  \\
& 2. &  Expected to be more robust to limited multimodal datasets used for end-task finetuning.\\
\midrule
\multirow{5}{*}{\emph{\color{myred} Cons}}       & 1. & Text inputs in multimodal pretraining dataset are often simple  language captions.   \\
& 2. & Joint models are smaller than PLMs. \\
& 3. & If captioning is only \emph{generative} pretrain task, they are \emph{not} designed for generation conditioned on \emph{both} images and text.  \\
& 4. & Requires training from scratch. \\
\bottomrule
\end{tabular}}
\caption{Summary of {\color{mygreen} pros} and {\color{myred} cons} of training vision and language (VL) jointly from scratch (e.g., \vlp) versus adapting pretrained language models (PLM) to visual features (e.g., \vatfive). Some models are combinations of these two approaches (\vltfive, \vlbart). See \sect{sec:models_background} for more information about these models.}
\label{tab:open_research_questions}
\end{table*}


==> tables/pretraining_data.tex <==
\begin{table*}[t]
\centering{
\resizebox{0.95\textwidth}{!}{  
\begin{tabular}{llll}
\toprule
 \textbf{Model} & \textbf{Pretraining Text}   & \textbf{Pretraining Images} & \textbf{Test set Overlap}  \\ 
\midrule
\vlp & Conceptual Captions & Conceptual Captions & None\\
%\gpv & MS COCO, VQA v2, RefCOCO+ & MS COCO & \esnlive, \vqax \\
\midrule
\vltfive and \vlbart & MS COCO, Visual Genome,  & MS COCO, Visual Genome  & \esnlive, \\
 &  VQA v2, GQA, Visual 7W &  & \vqax \\
\midrule
\vatfive & None & None & None\\
\bottomrule
\end{tabular}}
\caption{Overview of text and image datasets used for pretraining by the different models. Testset overlap shows overlap of \vcr, \esnlive, and \vqax with pretraining data. }
\label{tab:pretraining_data}}
\end{table*}
